Approximation and Kernelization for Chordal Vertex Deletion

The Chordal Vertex Deletion (ChVD) problem asks to delete a minimum number of vertices from an input graph to obtain a chordal graph. In this paper we develop a polynomial kernel for ChVD under the parameterization by the solution size, as well as poly(opt) approximation algorithm. The first result answers an open problem of Marx from 2006 [WG 2006, LNCS 4271, 37-48].

==> old-approximation.tex <==
This section is devoted to the proof of Theorem~\ref{thm:apx}.

First, in Section~\ref{s:apx:defs} we recall the definition
of the \multicut problem, and formally define LP relaxations
of \multicut and \ChVD. 
Subsequent two sections are devoted to approximation algorithms for \multicut
in two specific cases: \skewmc and \multicut in downwards oriented
chordal graphs (defined in Section~\ref{s:apx:mc}).
In Section~\ref{s:apx:clique} we focus on approximating
\ChVD in a special case of graphs $G$ where $V(G)$ partitions
into $A \uplus B$ such that $G[A]$ is chordal and $G[B]$ is complete.
Finally, we wrap up the approximation algorithm in Section~\ref{s:apx:final}.

\subsection{Multicut and LP relaxations}\label{s:apx:defs}

An instance to the \multicut problem consists of a directed graph $G$
and a family $\terms \subseteq V(G) \times V(G)$ of \emph{terminal pairs}.
A set $X \subseteq V(G)$ is a feasible solution to a multicut instance
$(G,\terms)$ if, for every $(s,t) \in \terms$, there is no path from 
$s$ to $t$ in $G-X$.
The \multicut problem asks for a feasible solution of minimum cardinality.
That is, we focus on unweighted node-deletion variant of \multicut,
and note that the set $X$ may contain terminals.

\multicut is NP-hard even in undirected graphs with three terminal
pairs~\cite{DahlhausJPSY94}. 
The best known approximation ratio for undirected graphs is $\Oh(\log n)$~\cite{GargVY96}, but for general directed graphs only $\Oh(\sqrt{n})$-approximation
is known~\cite{Gupta03}. 
Since the latter is insufficient for our purposes, in the next two sections
we develop approximation algorithms with better approximation guarantees
for specific cases of our interest.

Given a \multicut instance $(G,\terms)$, an \emph{LP relaxation} is
a function $\LPsol:V(G) \to [0,1]$ such that for every $(s,t) \in \terms$
and every path $P$ from $s$ to $t$ in $G$, we have
$$\LPsol(P) := \sum_{v \in V(P)} \LPsol(v) \geq 1.$$
The equation above is a linear constraint on values of $\LPsol$
that defines the polytope of LP relaxations. Clearly, a feasible solution
to the \multicut instance $(G,\terms)$ induces a LP relaxation that assigns
$1$ to the vertices of the solution. 
Furthermore, the separation oracle of 
the aforementioned polytope is straightforward to implement.
Consequently, using the ellipsoid method, in polynomial time
we can find a LP relaxation of total value arbitrarily close to minimum possible.

Very similarly we define an LP relaxation to \ChVD on an undirected graph $G$:
it is a function $\LPsol:V(G) \to [0,1]$ such that for every hole $H$
in $G$ we have
$$\LPsol(H) := \sum_{v \in V(H)} \LPsol(v) \geq 1.$$
Again, the equation above defines a polytope containing all feasible
solutions to \ChVD on $G$, and there is a simple separation oracle
for this polytope.\footnote{Iterate over all possibilities of three consecutive vertices $v_1,v_2,v_3$ on the hole $H$, and compute the shortest path from $v_1$ to $v_3$
in $G-N[v_2]$ with respect to the distances defined by the current values of $\LPsol$.}

\subsection{Approximating Skew Multicut}\label{s:apx:skew}

We first focus on a specific case of \multicut, namely \skewmc.
Here, we assume that the input $(G,\terms)$ additionally identifies two sets of terminals $T_u = \{u_1,u_2,\ldots,u_a\}$ and $T_v = \{v_1,v_2,\ldots,u_b\}$ with the following properties:
$\terms \subseteq T_v \times T_u$ and whenever $(u_i,v_j) \in \terms$, then
$(u_{\hat{i}},v_{\hat{j}}) \in \terms$ for every $\hat{i} \geq i$ and $\hat{j} \leq j$.
The main result of this section is the following.

\begin{lemma}\label{lem:apx:skewmc}
Given a \skewmc instance $(G,\terms)$ with terminal sets $T_u$ and $T_v$,
and its LP relaxation $\LPsol$, one can in polynomial time
compute a solution to $(G,\terms)$ of size at most 
$|\LPsol| \cdot \lceil \log (|T_u|+1) \rceil$.
\end{lemma}
\begin{proof}
For this proof, it is more convenient to switch to a variant of \multicut
and \skewmc where we are not allowed to delete terminals.
Formally, for every $u \in T_u$ we add a copy $u'$ and an arc $(u',u)$,
similarly for every $v \in T_v$ we add a copy $v'$ and an arc $(v,v')$,
and replace every pair $(u,v) \in \terms$ with $(u',v')$.
In the new instance, we seek for an integral solution disjoint with
$T_u \cup T_v$, and the LP relaxation $\LPsol$ assigns value $0$
to every new terminal $u'$ or $v'$.

We use induction on $|T_u|$. For $T_u = \emptyset$ there is nothing to prove.
For $T_u = \{u_1\}$, the instance $(G,\terms)$ can be reduced to an instance
of the minimum cut problem, and thus a solution of size at most $|\LPsol|$
can be found in polynomial time.

Assume then $a = |T_u| \geq 2$. Define $T_u^1 = \{u_1,u_2,\ldots,u_{\lfloor a/2 \rfloor}\}$ and $T_u^2 = T_u \setminus T_u^1$.
Let $i := \lfloor a/2 \rfloor + 1$ and let $j$ be largest index such that $(u_i,v_j) \in \terms$;
we have $0 \leq j \leq b$.
Let $T_v^1 = \{v_1,v_2,\ldots,v_j\}$ and $T_v^2 = T_v \setminus T_v^1$.

We now note two consequences the definition of \skewmc.
First, since $(u_i,v_j) \in \terms$ (or $j=0$ and then $T_v^1 = \emptyset$),
we have $T_u^2 \times T_v^1 \subseteq \terms$.
Second, since $(u_i,v_{j+1}) \notin \terms$ (or $j=b$ and then $T_v^2 = \emptyset$),
we have $T_u^1 \times T_v^2 \cap \terms = \emptyset$.

The first consequence implies that a minimum cut $X^0$ between $T_u^2$ and $T_v^1$
is of size at most $|\LPsol|$. 
With the second consequence, we can decompose
$$\terms = (T_u^2 \times T_v^1) \uplus \terms^1 \uplus \terms^2,$$
where
\begin{align*}
\terms^1 &= \terms \cap (T_u^1 \times T_v^1)\\
\terms^2 &= \terms \cap (T_u^2 \times T_v^2)
\end{align*}
Let $A^1 \subseteq V(G) \setminus X^0$ be the set of vertices
from which we can reach $T_v^1$ in $G-X^0$,
and let $A^2 \subseteq V(G) \setminus X^0$ be the set of vertices
reachable from $T_u^2$ in $G-X^0$. Since $X^0$ is a cut between $T_u^2$
and $T_v^1$, we have $A^1 \cap A^2 = \emptyset$.
Furthermore, note that for every $i=1,2$, 
for every $(u,v) \in \terms^1$, and for every path $P$ from $u$ to 
$v$ in $G-X^0$, every vertex on $P$ lies in $A^i$.

Consequently, $\LPsol|_{A^i}$ is an LP relaxation to \skewmc
instance $(G[A^i],\terms^i)$.
For $i=1,2$, we recursively solve the instance $(G[A^i],\terms^i)$
with LP relaxation $\LPsol|_{A^i}$, obtaining a solution $X^i$.
We output a solution $X := X^0 \cup X^1 \cup X^2$.
It is immediate from the previous observations that $X$
is a solution to \skewmc on $(G,\terms)$.
Furthermore,
\begin{align*}
|X| &= |X^0| + |X^1| + |X^2| \leq |\LPsol| +
 \left|\LPsol|_{A^1}\right| \left\lceil \log\left(|T_u^1| + 1\right) \right\rceil +
 \left|\LPsol|_{A^2}\right| \left\lceil \log\left(|T_u^2| + 1\right) \right\rceil\\
 &\leq |\LPsol| + \left(\left|\LPsol|_{A^1}\right| + \left|\LPsol|_{A^2}\right|\right) \left(\lceil\log(|T_u|+1)\rceil - 1\right) \\
 &\leq |\LPsol| + |\LPsol|\left(\lceil\log(|T_u|+1)\rceil - 1\right) = |\LPsol|\lceil\log(|T_u|+1)\rceil.
\end{align*}
\end{proof}

\subsection{Approximating Multicut in downwards oriented chordal graphs}\label{s:apx:mc}

Assume we are given a chordal graph $G$, together with its clique tree $(T,\beta)$
rooted in a node $\root \in V(T)$. 
We define a partial order $\preceq_0$ on $V(G)$ as $v \prec_0 u$ for $v,u \in V(G)$
iff $\top(v)$
is an ancestor of $\top(u)$ in $T$. We fix any total order $\preceq$
extending $\preceq_0$.
Furthermore, we define an orientation $\Gdown$ of $G$ as follows:
an edge $uv \in E(G)$ is oriented as $(u,v)$ iff $u \prec v$.
Note that $\Gdown$ is a directed acyclic graph, and $\preceq$ is
its topological ordering.

The main result of this section is an approximation algorithm for
\multicut on graphs $\Gdown$ defined as above.
\begin{lemma}\label{lem:apx:mc}
Given a \multicut instance $(\Gdown,\terms)$, where $\Gdown$ is defined
as above, and its LP relaxation $\LPsol$, one can in polynomial time
compute an integral solution to $(\Gdown,\terms)$ of
size $\Oh(|\LPsol|^2 \log n)$, where $n = |V(\Gdown)|$.
\end{lemma}
\begin{proof}
We first consider the set $X^0 = \{v \in V(G): \LPsol(v) \geq 1/8\}$.
Clearly, $|X^0| \leq 8|\LPsol|$. We put $X^0$ into the solution we are looking
for, and delete $X^0$ from the graph $\Gdown$.
Consequently, we can from this point assume that $\LPsol(v) < 1/8$
for every $v \in V(\Gdown)$.

Let $G$, $(T,\beta)$, $\root$, $\preceq_0$, and $\preceq$ be as in the definition
of $\Gdown$.
Let $(u,v) \in \terms$.
First, we can assume that there 
is at least one $uv$-path in $\Gdown$, as otherwise we can 
delete $(u,v)$ from $\terms$. This in particular implies that $u \preceq v$.
Furthermore, since $\LPsol(v) < 1/8$ for every $v \in V(G)$, every $uv$-path
in $\Gdown$ constains at least $9$ vertices. In particular,
$uv \notin E(G)$, that is, $\binv(u) \cap \binv(v) = \emptyset$.
By the definition of $\Gdown$, we infer that the path $\MPtd(u,v)$
is contained in $\MPtd(v,\root)$. Let $T_{u,v}$ be the set of
internal vertices of $\MPtd(u,v)$.
Moreover, let $P_{u,v}$
be a shortest (in terms of the number of vertices) $uv$-path in $\Gdown$,
and let $A_{u,v}$ be the set $V(P_{u,v})$ except for the first two
and the last two vertices of $P_{u,v}$.

We construct an auxiliary graph $H$ with $V(H) = \terms$;
two terminal pairs $p,q \in \terms$ are adjacent in $H$ if $T_p \cap T_q \neq \emptyset$. 
Since $T_p \subseteq V(T)$ and $T[T_p]$ is a path, $H$ is a chordal graph.
Furthermore, we have the following claim:
\begin{claim}\label{cl:apx:mc1}
If $p,q \in \terms$ and $pq \notin E(H)$, then $A_p \cap A_q = \emptyset$.
\end{claim}
\begin{claimproof}
Let $p = (u_p,v_p)$ and $q = (u_q,v_q)$.
Recall that $T[T_p]$ (and similarly $T[T_q]$)
 is a path in $T$ that is contained in some leaf-to-root path. 
Let $e_p$ be the edge of $T$ connecting $T[T_p]$ and $T[\binv(u_p)]$,
and similarly define $e_q$.
That is, $e_p$ is the edge from the topmost vertex of $T_p$ to its parent.
Since $T_p \cap T_q = \emptyset$, either $e_p$ or $e_q$ separates
$T_p$ from $T_q$; by symmetry, assume that $T_p$ and $T_q$ lie in different
connected components of $T-e_p$.

Since $P_p$ is a shortest $u_pv_p$-path, for every internal vertex $w$
of this path we have $\binv(w) \cap A_p = \emptyset$. A similar
claim holds for $P_q$. Furthermore, we infer that 
all vertices of $A_p$ are nonadjacent
to $u_p$ in $G$: if some $w \in A_p$ was adjacent to $u_p$,
then $(u_p,w) \in E(\Gdown)$ as $u_p \preceq w$, and we could have
shortened the path $P_p$.
Consequently, for every $w \in A_p$, the set
$\binv(w)$ is contained in the connected component of $T-e_p$
containing $T_p$. In particular, $\binv(w) \cap T_q = \emptyset$,
and thus $w \notin A_q$. This finishes the proof of the claim.
\end{claimproof}
Consider now an independent set $\terms_I \subseteq \terms$ in $H$.
By Claim~\ref{cl:apx:mc1}, the sets $A_p$ for $p \in \terms_I$ are pairwise
disjoint.
Consequently, if $|\terms_I| \geq 2|\LPsol|$, there exists a pair $p \in \terms_I$
with $\LPsol(A_p) \leq 1/2$.
On the other hand, $\LPsol(P_p) \geq 1$. This is in contradiction
with the assumption that $\LPsol(v) < 1/8$ for every $v \in V(G)$,
as $V(P_p) \setminus A_p$ contains at most four vertices.

We infer that the size of the largest independent set in $H$ is of size
smaller than $2|\LPsol|$. Since $H$ is a chordal graph, $V(H)$ can be partitioned
into $\ell < 2|\LPsol|$ parts $\terms_i$,
such that $H[\terms_i]$ is complete for every $1 \leq i \leq \ell$.
Our goal for the rest of this proof is to provide an integral solution $X_i$
of size $\Oh(|\LPsol| \log n)$ to every instance $(\Gdown,\terms_i)$;
by taking the union of all solutions $X_i$ we obtain the desired solution
to $(\Gdown,\terms)$.

Fix an index $1 \leq i \leq \ell$. Since $H[\terms_i]$ is a complete graph, there
exists a node $s \in \bigcap_{p \in \terms_i} T_p$.
For a pair $p = (u,v) \in \terms_i$, we define
$$\beta_p := \{w \in \beta(s): u \preceq w\}.$$
Since $u,v \notin \beta(s)$, every $uv$-path in $\Gdown$ contains a vertex
of $\beta(s)$; by the definition of $\Gdown$, this vertex actually needs
to belong to $\beta_p$.

We now look at $\Gdown$ with distances measured with respect to the LP
relaxation $\LPsol$. That is, for two vertices $u,v \in V(\Gdown)$,
by $\dist_{\LPsol}(u,v)$ we mean the minimum cost of a $uv$-path in $\Gdown$,
where the cost of traversing a vertex $w$ is $\LPsol(w)$.
We observe the following.
\begin{claim}\label{cl:apx:mc2}
For every $p = (u,v) \in \terms_i$ it holds that
$$\dist_{\LPsol}(u,\beta(s)) + \dist_{\LPsol}(\beta_p,v) \geq 1.$$
\end{claim}
\begin{claimproof}
Assume the inequality does not hold for a pair $p = (u,v)$.
Let $P_1$ be a $uw_1$-path for some $w_1 \in \beta(s)$
and $P_2$ be a $w_2v$-path for some $w_2 \in \beta_p$,
such that $\LPsol(P_1) + \LPsol(P_2) < 1$.
Let $w$ be the last vertex on $P_1$ with $w \preceq w_2$;
such a vertex exists since $u \preceq w_2$.
If $ww_2 \in E(G)$, then the concatenation of the subpath of $P_1$ from $u$ to $w$
and the $P_2$ gives
a $uv$-walk in $\Gdown$ of cost (w.r.t. $\LPsol$) less than $1$, a contradiction.
Hence, $ww_2 \notin E(G)$, in particular $w \neq w_1$.

Let $w'$ be the vertex after $w$ on $P_1$. By the definition of $w$,
we have $w_2 \preceq w'$. Since both $\binv(w')$ and $\binv(w_2)$ contain
nodes of $\MPtd(s,\root)$, this implies that $\top(w')$ is equal to or is 
a descendant of $\top(w_2)$. However, $w \preceq w_2$ and $ww' \in E(G)$
implies that $w \in \beta(\top(w_2))$, a contradiction to the fact
that $ww_2 \notin E(G)$.
\end{claimproof}
We partition $\terms_i$ into two parts $\terms_i^\uparrow$ and $\terms_i^\downarrow$:
we assing $p=(u,v)$ to $\terms_i^\uparrow$ if $\dist_{\LPsol}(u,\beta(s)) \geq 1/2$
and to $\terms_i^\downarrow$ otherwise.
Note that Claim~\ref{cl:apx:mc2} implies that for every $p=(u,v) \in \terms_i^\downarrow$ we have $\dist_{\LPsol}(\beta_p,v) \geq 1/2$.
We now separatedly solve \multicut instances
$(\Gdown,\terms_i^\uparrow)$ and $(\Gdown,\terms_i^\downarrow)$.

For the first instance, note that $2\LPsol$ is contained in a polytope
for a minimum cut between $\{u : (u,v) \in \terms_i^\uparrow\}$ and $\beta(s)$.
That is, a minimum cut between $\{u: (u,v) \in \terms_i^\uparrow\}$
and $\beta(s)$ is of size at most $2|\LPsol|$.
Consequently, we can add such a minimum cut to the constructed solution,
cutting all terminal pairs from $\terms_i^\uparrow$.

For the second instance, we order $\beta(s)$ according to
$\preceq$, that is, $\beta(s) = \{w_1,w_2,\ldots,w_k\}$
with $w_1 \preceq w_2 \preceq \ldots \preceq w_k$.
Similarly, we order $\terms_i^{\downarrow}$ according to $\preceq$
on terminals $u$, that is, $\terms_i^{\downarrow} = \{p_1,p_2,\ldots,p_\ell\}$
with $p_j = (u_j,v_j)$ and $u_1 \preceq u_2 \preceq \ldots \preceq u_\ell$.
We define
$$\terms_i^{\downarrow w} := \bigcup_{p=(u,v) \in \terms_i^\downarrow} \beta_p \times \{v\}$$
and observe the following:
\begin{claim}\label{cl:apx:mc3}
$(\Gdown,\terms_i^{\downarrow w})$ is a \skewmc instance
with the aforementioned orders $w_1,w_2,\ldots,w_k$ and $v_1,v_2,\ldots,v_\ell$.
\end{claim}
\begin{claimproof}
The claim follows from the definition of $\terms_i^{\downarrow w}$
and the observation that for $j \leq \hat{j}$, since $u_j \preceq u_{\hat{j}}$, we have $\beta_{p_j} \supseteq \beta_{p_{\hat{j}}}$. 
\end{claimproof}
By the definition of $\terms_i^{\uparrow}$, $2\LPsol$ is an LP relaxation
to the instance $(\Gdown,\terms_i^{\downarrow w})$.
By Lemma~\ref{lem:apx:skewmc}, we can compute a solution
to $(\Gdown,\terms_i^{\downarrow w})$ of size $\Oh(|\LPsol| \log n)$.
Since for every $p = (u,v) \in \terms_i$, every $uv$-path constains
a vertes of $\beta_p$, a solution to $(\Gdown,\terms_i^{\downarrow w})$
is also a solution to $(\Gdown,\terms_i^{\downarrow})$.
This concludes the proof of the lemma.
\end{proof}

\subsection{Adding a clique to a chordal graph}\label{s:apx:clique}

\subsection{The approximation algorithm}\label{s:apx:final}

